3D-NVS: A 3D Supervision Approach for Next View Selection

We present a classification based approach for the next best view selection and show how we can plausibly obtain a supervisory signal for this task. The proposed approach is end-to-end trainable and aims to get the best possible 3D reconstruction quality with a pair of passively acquired 2D views. The proposed model consists of two stages: a classifier and a reconstructor network trained jointly via the indirect 3D supervision from ground truth voxels. While testing, the proposed method assumes no prior knowledge of the underlying 3D shape for selecting the next best view. We demonstrate the proposed method's effectiveness via detailed experiments on synthetic and real images and show how it provides improved reconstruction quality than the existing state of the art 3D reconstruction and the next best view prediction techniques.

==> sections/conclusion.tex <==
\section{Conclusion}
In this paper, we present how the task of Next Best View prediction can be posed as a classification problem and learned in a data driven manner without the knowledge of underlying ground truth labels.
We do this with an aim to obtain the best possible 3D reconstruction from the acquired views and use this reconstruction process to obtain an indirect supervision to train the proposed model.
The performance of the proposed 3D-NVS method is evaluated on both synthetic and real data to demonstrate how it obtains better reconstruction quality than the existing state of the art 3D reconstruction techniques by effectively selecting the best view.
Additionally, we present an analysis of how the NBV locations are distributed intuitively depending on the object category which concurs with previous techniques that use range sensors.
Going forward we aim to extend this to successive N-view next view selection.

% Going forward we plan to extend 3D-NVS to accommodate successive N-view selection. For example, if base image selects a next view, we use these two inputs and predict the third view and so on. One of the challenges associated with this generalization is that after a few views, the performance is essentially equal to random selection of N views. Consequently, the reconstruction performance is also the same.

% We also plan to incorporate differential rendering \blue{cite} that would enable us to render images on the fly and predict the next views based on that. Such an experiment can also be combined with quantitative results on robotics or UAV simulator.
% \sk{I think there is no need to mention Future work as their it is of no use in the paper untill it's done. Also, it is rarely found in vision papers plus lets the ideas out if the plan it to actually do them later. One para conclusions is all there is typically.}

%Going forward we plan to extend this to:
%\begin{itemize}
%    \item N stage NBV?
%    \item quantitative results on robotics or UAV simulator.
%    \item Something else / or some other application?
%\end{itemize}

==> sections/figs_and_tables.tex <==




==> sections/introduction.tex <==
\section{Introduction}
Three dimensional (3D) object reconstruction and acquisition are a long time focus of machine vision research and a key to visual understanding and interpretation.
It has a wide range of practical applications including robotics, AR/VR, autonomous navigation and industrial automation to name just a few.
Being able to access the 3D geometric cue about an object or scene can immensely benefit in post processing and decision making for instance in recognition \cite{pontil1998support}, segmentation \cite{qi2017pointnet}, pose estimation \cite{andriluka2010monocular} and other computer vision and pattern recognition tasks.

As a computer vision task, this requires a sensor for observing the object which can be of two types namely, active and passive cameras.
Active cameras like Laser iamging detection and ranging (LiDAR), Time of Flight (ToF) and depth cameras like the Kinect directly acquire scene depth and in turn the 3D shape of an object but come with their own limitations apart from the high cost and power requirements.
Passive cameras are much cheaper and use significantly less power to acquire two dimensional (2D) optical RGB snapshots of the object which can then be used to recover the 3D structure by posing this as an inverse problem.

Recovering 3D shape from its two dimensional snapshots has been a goal of classic computer vision problems like multiview stereo and Shape-from-X techniques.
Early methods approached this with a geometric perspective and focussed on mathematically modelling the process of 2D projection to pose it as an ill-posed problem \cite{hartley2003multiple} constrained by suitable scene priors.
The structure from motion(SfM) techniques can be used to obtain a sparse 3D point cloud of an object along with the respective camera poses.
Along the similar lines, Multi View Stereo (MVS) techniques can provide a dense 3D reconstruction.
Recently, with the advent of deep learning based methods, a model can directly learn a non linear mapping from the images to the 3D representation outperforming classical methods while doing it in real time \cite{pix2vox}.

% MVS to NBV
Although, there are works which attempt to reconstruct the 3D shape of an object from just a single view but these are in early stages due to their highly ill posed nature of the problem.
Moreover, as in MVS, taking more than one view of the object reduces ambiguity and occlusion to significantly improve the 3D recognition quality as more information is available for recovery.
Typically, these views are acquired from a set of passively selected viewpoints independent of the object geometry.
In order to obtain the best 3D reconstruction, one would expect the location of these viewpoints to be dependent on the 3D shape in consideration.
Therefore, to obtain the best possible 3D reconstruction quality from the captured images one has to actively decide the next best view point to take the snapshot from.

% Motivation and Intro to NBV
The Next View Selection (NVS) problem has been explored since the early days of machine vision research \cite{connolly1985determination}.
This problem arises in many scenarios where one would want to find the next best viewpoint around an object or in an arena while maximizing a certain quality or performance metric.
For instance, in order to better grasp an object, a robotic arm equiped with a camera may want to find the next viewpoint to obtain the best 3D reconstruction for better understanding quickly.
Similarly, a UAV hovering over a scene may want to find the next view which can provide the best 3D digital elevation model in order to minimize the flight time.
There are several works in robotic navigation, robotic arm positioning and remote sensing which are discussed in the related work section.

% Gaps in the literature, typically done and what they lack
However, almost all of these works use range cameras to directly capture scene depth and select the next view either heuristically or by optimizing for the suface area covered or information gained.
Along with this, their aim has been to reconstruct a surface representation of the scene like mesh or point cloud.
Volumetric representation like voxels are better suited for practical applications due to ease of manipulation and training than surface or mesh based representations.
Hence, we focus on learning a volumetric representation of the scene in this work.
Moreover, selecting next views using only passive camera images of a scene has been explored much recently but not very actively in the literature and we focus on this particular setup in this paper.
Predicting a 3D shape or next views using passive cameras is a more challenging task due to much lesser data available for use than in the case of active sensors.
Due to this setup of the problem, classical solutions based on surface reconstruction and optimized for surface area covered or information gained cannot be used here.

% A hint of advantages of the proposed method and how it fits into the bigger picture
In this paper, we attempt to address these gaps and propose a novel classfication based approach for NVS without using the preprocessed ground truth next views.
Since our goal is to maximize the 3D reconstruction quality, we propose to extract supervisory signal from the reconstruction process itself to to drive the training of classifcation model and hence obtain a better loss-goal correspondence.
We present how a light-weight neural network based classifier can be incorporated into existing 3D reconstruction models to perform NVS and trained without the knowledge of ground truth NVS labels.
Training such a classifier-reconstructor architecture is not straightforward without the labels and therefore we propose a novel loss objective that facilitates end to end training of such a joint classifier-reconstructor deep neural network model.

% End with a hint of some key findings and insights gained
We demonstrate how the proposed method successfully selects the next views that maximize the reconstruction quality for a given 3D object on both synthetic and real data.
Additionally we analyse the NBVs predicted for each object category to gain insights and observe underlying patterns to learn how they are distributed depending on the object shape.
Our contributions in this paper are as follows:
\begin{itemize}
    \item We propose a deep learning based approach for next view selection and show how it can be effectively approached as a classifcation problem.
    \item We show how the supervisory signal form the 3D reconstruction process can be used to learn both the classfication and reconstruction networks jointly in an end to end manner.
    \item We present a qualitative analysis of the NBV predictions to gain insights into the process and their dependence on object categories and shape.
    \item We present exhaustive experiments on both synthetic and real data to demonstrate the effectiveness of the proposed method in selecting appropriate NBV while providing high reconstruction quality.
\end{itemize}


\begin{figure*}
\begin{center}
\includegraphics[scale=0.36]{figures/3d-nvs-overview.pdf}
\end{center}
   \caption{An Overview of the proposed 3D-NVS model used during the (a) training and (b) testing. A detailed explanation of each sub-parts is given in Section \ref{sec:method}. (c) Chosen viewpoints of the ShapeNet dataset to generate images for training.}
\label{fig:overview-model}
\end{figure*}

==> sections/method.tex <==
\section{Method}
\label{sec:method}
%\begin{figure*}
%\begin{center}
%\includegraphics[scale=0.37]{figures/fig_draft.pdf}
%\end{center}
%   \caption{Draft 1 of Model Schematic Diagram}
%\label{fig:short}
%\end{figure*}
%This section is dedicated for the method section.
In this section, we introduce 3D-NVS -- a novel deep learning model to reconstruct 3D shape from 2D images while selecting the best next view. The proposed two-stage model works as follows: given an input image, the stage 1 selects the next camera position out of 11 possible labels and subsequently, stage 2 inputs the two images (base image and the selected next view) to a reconstruction model to generate a 3D shape. The shape is in the form of voxel grids with binary occupancy (1 means occupied, 0 means empty). To select the next views, 3D-NVS uses supervision from ground truth 3D shapes. This indirect supervision is facilitated by a novel loss function which enables training of a network with a softmax classifier in between. Such a unified classifier followed by reconstruction architecture is the first in our knowledge and is a key enabler of our proposed method. An overview of the proposed model is presented in Figure \ref{fig:overview-model} and the detailed architecture is shown in Figure \ref{fig:model-architecture}.
\subsection{Network Architecture}
We use slightly different architectures for training and testing. For training, we incorporate the availability of images from all camera viewpoints. However, during testing, we only input image from any one viewpoint and the model predicts the next-best view. This idea reinforces the freedom of obtaining multiple images from all viewpoints during training while restricted access during testing. %\ka{TODO: Write that this is inspired from GAN}
%\sk{It will be better to explain this with a figure and we can have two larger outer blocks / other indicators that house the two stages and name them as done in next para class-net, core (houses the encoder-decoder pair) and refiner and then explain this by referring to that figure.}

During training, the input RGB image from arbitrary camera position, called henceforth as base image, is passed into NVS-Net which outputs a probability distribution over the next views. The number of possible camera positions for the next view is fixed (details in Section \ref{sec:experiments}) and thus, is a classification problem. In parallel to NVS-Net, we pass images from all the viewpoints into the Encoder -- a sub-network of Stage 2 of 3D-NVS, that generate feature maps. These are then used by the Decoder to produces coarse voxels. The context-aware fusion and the refiner \cite{pix2vox} are used to further fine-tune the generated voxels. The 3D volumes obtained from all pairs of base image and possible next-best views are combined with the probability distribution predicted by the NVS-Net to obtain a final 3D volume.

During testing, we simply detach the stage 1, that is NVS-Net from the training setup \& use it for next view selection described above and predicts the probability distribution over next views. Now, the viewpoint with maximum probability is selected as the next view and the two views (base view and selected next view) are passed into the Encoder, Decoder, Context-aware Fusion and Refiner sub-networks to obtain the final reconstructed 3D volume.
\subsubsection{NVS-Net}
We use a classification network inspired by VGG16 \cite{vgg} and modify the last few layers of this network to suit our output classes. We take the model pre-trained on ImageNet \cite{imagenet} and freeze first nine layers. An RGB square input image of size 228 pixels is progressively passed into convolutional layers with ELU activations while increasing the number of channels as described in Figure \ref{fig:model-architecture}. Finally, we obtain a 256x4x4 feature map which is flattened into a 4096 dimensional fully-connected layer and fed to two further fully-connected layers output 128 and 11 channel outputs, respectively. The activation of the last layer is set to softmax to obtain probability distribution over next views, as in other standard classification models.

In the remainder of the paper, we define 3D-NVS-R as the model where we choose the next view randomly from all the available views. In addition, we define 3D-NVS-II when we choose the second best view, 3D-NVS-III for the third view and so on. Finally, 3D-NVS-F is when the next view is choosen so as the maximize the distance between the pair of input images.
\subsubsection{Encoder-Decoder}
The encoder extracts features from both input RGB images, the base and next view image selected by NVS-Net. Since the NVS-Net already extracts features and flattens them for classification, we share its parameters with Encoder for parameter efficiency and smaller model. The output of the Encoder is a feature map of size 256x8x8 which is an intermediate output of NVS-Net. Note that only the base image is passed into the NVS-Net, whereas all the images are passed into the Encoder in stage 2 during the training phase.

After obtaining the feature maps, we use those as input to recover 3D shapes. The architecture of having an Encoder-Decoder model is motivated by its success in Image Segmentation tasks \cite{7803544} and to more related 3D shape reconstruction tasks \cite{pix2vox}. The feature maps of size 256x8x8 is resized to 2048x2x2 and operated on successive transposed convolution layers that decreases the number of channels and increases the feature sizes. The obtained 32x32x32 vector is passed through a sigmoid activation function to obtain occupancy probability for each cell.
\subsubsection{Context-aware Fusion and Refiner}
Context-aware Fusion and Refiner is used in Pix2Vox \cite{pix2vox}  to convert coarse 3D volumes into an improved 3D volume. The idea behind such an additional network is to account for different reconstructions from different viewpoints. The Context-Aware Fusion generates a score map based on the viewpoint and the final volume is obtained by multiplying a softmax-based activation with the corresponding coarse volume from that view. Finally, the Refiner is a UNet-like architecture \cite{unet} which acts as a residual network to correct remaining mis-recovered parts of the object. The activation of the final layer is again set to sigmoid to obtain occupancy probability for the 32x32x32 grid.
\subsubsection{Loss Function}
We propose a loss function to train this unique architecture. The proposed loss function considers both NVS-Net output probability and the reconstructed 3D shape for each pair of views. Let the probability of selecting $i^{th}$ image is $p_i$ as per NVS-Net. Correspondingly, let $v_i$ denote the reconstructed volume of size 32x32x32 using base image and $i^{th}$ image as input. The averaged 3D shape is defined as 
\begin{equation}
    r = \sum_{\forall i} p_i v_i
\end{equation}
We propose the averaged per-voxel binary cross entropy between $r$ and ground truth voxel $t$ as the loss function of the network. Mathematically,
\begin{equation}
    L(r, t) = \frac{1}{N} \sum_{j=1}^{N} (t_j\log(r_j) + (1-t_j)\log(1-r_j))
\end{equation}
It is advantageous to have output from both the sub-networks in the expression of the loss. Such a choice prevents a network weight bottleneck at the NVS-Net outputs and serves the objective of simultaneous classification and reconstruction tasks. Our motivation to use this loss function is to improve the weighted reconstruction, that is, at each training step, we aim to improve the reconstruction performance on the network. Once it is trained successfully, the NVS-Net is inclined to assign a higher weight to the view which has a lower loss thus achieving our two-fold objectives of Next View Selection and reconstruction.


==> sections/relatedwork.tex <==
\section{Related Work}
%\ka{We should also mention the weakness of using very narrow camera position. For example, in some applications like UAV or underwater imaging it is desirable to be able to take images from a wider area. Also, some points on why a spread-out camera position is better than fixed elevation images despite a decrease in reconstruction performance}
%\sk{Certainly, we can maybe push this to intro to highlight the gaps in literature? Can you write up a gist for this along with a reason for why specifically in underwater and UAV imaging?} 
%\ka{I will add this in the dataset section}
% \subsection{3D Reconstruction}

% Classical methods

% Deep learning based
Early works on 3D reconstruction focus on mathematically modeling the imaging process and solving an ill posed problem via suitable scene priors and geometric constraints \cite{hartley2003multiple}.
Among the recent deep learning based methods, there are three broad types of techniques based on the choice of output representation :
Volume-based, Surface-based and Intermediate representation.
Surface based methods explore meshes and point clouds that are unordered representations \cite{wang2018pixel2mesh, kanazawa2018learning, pontes2018image2mesh}. 
Volumetric methods explore regular voxel grid based representation as we consider in this paper \cite{wu2017marrnet, tulsiani2017multi, yang2018learning}.
The recent state of the art works in this category include Pix3D \cite{sun2018pix3d}, 3DR2N2 \cite{3dr2n2} and Pix2Vox \cite{pix2vox} which we use as our baselines to compare with.
There are also techniques that decompose the problem into sequential steps each predicting a different representation that can be used as per application \cite{tatarchenko2016multi, lin2018learning}.

% \subsection{Next View Selection}

% Use active cameras
Early works in NVS acquire range images and aim to recover surface geometry of an object.
Connolly et al. \cite{connolly1985determination} did one of the first works on automatic range sensor positioning using partial octree models and optimize for surface area covered.
Maver et al. employ occlusion guidance \cite{maver1993occlusions} and optimize for information gained \cite{maver1993planning} for NVS.
These and related methods \cite{pito1996sensor, pito1995solution, pito1999solution} require the images to have an overlap to allow for registration and integration of the new data captured with previous scans. 
Earliest work in data driven NVS is by Banta et al. \cite{banta1995best} which use synthetic range data to predict occupancy grids.
Here, the number of viewpoints on the view sphere are limited and the radius is large enough to encompass the whole object.
The center and coordinate axes of the view sphere are aligned with those of the object and the camera always faces this centre.
We work with a similar setup but use passive RGB cameras.

Recent works also focus on active sensors such as Hepp et al. \cite{hepp2018learn} use a CNN to learn a viewpoint utility function, Delmarico et al. \cite{delmerico2018comparison} optimize volumetric infromation gain and Mendez et al. \cite{mendez2017taking} maximize information gain in terms of total map coverage and reconstruction quality.
Chen et al. \cite{chen2005vision} propose a prediction model for the unknown area of the object using a 3D range data acquisition.
Zhang et al. \cite{delmerico2018comparison} use self oclusion information for NVS to predict 3D motion estimation.
Potthast et al. \cite{potthast2014probabilistic} and Isler et al. \cite{isler2016information} propose information gain based NVS for occluded enviroments and 3D reconstruction respectively.
Other works include greedy \cite{obwald2018gpu} and supervised learning approach \cite{ly2019autonomous} for visibility based exploration and reconstruction 3D enviroments.
Hashim et al. \cite{hashim2019next} propose a view selection recommendation method by minimizing pose ambiguity for object pose estimation using depth sensors.
There are also works on robotic arm navigation for autonomous exploration and grasping \cite{monica2018contour, morrison2019multi, bai2017toward, wu2019plant}, UAV positioning in remote sensing \cite{almadhoun2019guided}, Pose estimation \cite{sock2017multi} and 3D scene inpainting \cite{han2019deep}.

\begin{figure*}
\begin{center}
\includegraphics[scale=0.43]{figures/cvpr_architecture_final.pdf}
\end{center}
   \caption{The proposed 3D-NVS architecture showing various constituent stages: NVS-Net, Encoder, Decoder and Refiner modules. Note that Encoder shares weight with NVS-Net in the 3D-NVS model.}
\label{fig:model-architecture}
\end{figure*}

Closely related to our work and among the deep learning based methods, Wu et all. \cite{wu20153d} propose a deep neural network based view prediction but use 2.5D RGB-D images to improve 3D object recognition.
Daudelin et al. \cite{daudelin2017adaptable} propose a probabilistic NVS algorithm but use RGB-D sensor data for 3D object reconstruction.
Mendez et al. \cite{mendez2016next} use stereo image pairs and propose NVS to optimize for surface area covered by reconstructing object surface.
Dunn et al. \cite{dunn2009next} use passive cameras but optimize for surface area covered as their goal is surface reconstruction.
Mendoza et al. \cite{mendoza2020supervised} also pose the this as a classification problem but work with range sensor data and generate an exhaustive ground truth best view data to train a classifier.
They use a small dataset of 12 objects and CNN based classfier which takes the partial voxels as input to predict the next view. 
In contrast, we use RGB images and do not generate the ground truth but propose a classification based approach which is guided by the supervision from 3D reconstruction directly.
Yang et al. \cite{yang2018active} propose a recurrent network for NBV prediction using passive cameras but use a highly restricted set of viewpoints on the view sphere unlike the broad viewpoints considered in NBV literature and restrained acquisition process.


==> sections/results.tex <==
\section{Experiments and Observations}
\label{sec:experiments}
We conduct experiments with the proposed model on both synthetic dataset and real images. The details of dataset, implementations and observations are presented in next sub-sections.

\begin{table*}
\begin{center}
{\renewcommand{\arraystretch}{1.1} 
\begin{tabular}{P{0.14\textwidth}P{0.14\textwidth}P{0.14\textwidth}P{0.14\textwidth}P{0.14\textwidth}P{0.14\textwidth}}
\hline
Category & 3D-R2N2 \cite{3dr2n2} & Pix2Vox \cite{pix2vox} & 3D-NVS & 3D-NVS-R & 3D-NVS-F\\
\hline
airplane (810) & 0.486 & 0.619 & \textbf{0.627} & 0.418 & 0.384\\
bench (364) & 0.336 & 0.442 & \textbf{0.522} & 0.345 & 0.311\\
cabinet (315) & 0.645 & \textbf{0.709} & 0.656 & 0.619 & 0.595\\
car (1501) & 0.781 & 0.815 & \textbf{0.836} & 0.740 & 0.730\\
chair (1357) & 0.410 & 0.473 & \textbf{0.526} & 0.362 & 0.306\\
display (220) & 0.433 & \textbf{0.508} & \textbf{0.508} & 0.416 & 0.402\\
lamp (465) & 0.272 & 0.365 & \textbf{0.370} & 0.318 & 0.299\\
speaker (325) & 0.619 & \textbf{0.649} & 0.631 & 0.585 & 0.583\\
rifle (475) & 0.508 & \textbf{0.597} & 0.579 & 0.387 & 0.344\\
sofa (635) & 0.568 & 0.602 & \textbf{0.640} & 0.503 & 0.456\\
table (1703) & 0.405 & 0.438 & \textbf{0.510} & 0.343 & 0.293\\
telephone (211) & 0.636 & \textbf{0.818} & 0.681 & 0.628 & 0.700\\
watercraft (389) & 0.477 & 0.529 & \textbf{0.553} & 0.428 & 0.387\\
\hline 
Overall (8770) & 0.511 & 0.574 & \textbf{0.601} & 0.465 & 0.432\\
\hline
\end{tabular}
}
\end{center}
\caption{Class-wise comparison between state of the art reconstruction methods and our proposed 3D-NVS. Details of the experiment are described in Section \ref{sec:synthetic-results}. We also compare 3D-NVS-R and 3D-NVS-F with 3D-NVS, details of which is included in Ablation Study (see Section \ref{sec:ablation}). We can observe that 3D-NVS has the best overall reconstruction IoU amongst previous reconstrution and NVS works.}
\label{tab:result}
\end{table*}

\subsection{Dataset}
\label{sec:dataset}
ShapeNet \cite{shapenet} is a large-scale dataset containing 3D CAD models of common objects. We use a subset of ShapeNet with 13 categories having 43,782 models. This subset choice is same as that used in \cite{3dr2n2, pix2vox, yang2018active}. The 3D models are voxelized into 32x32x32 grid using the binvox package \cite{binvox, nooruddin03}. However, the rendered images for previous work \cite{pix2vox, 3dr2n2, yang2018active} positions the camera only on a circular trajectory over a fixed elevation (25$^\circ$ -- 30$^\circ$). Such highly-constrained acquisition of images is not particularly applicable to real-world acquisition followed by reconstruction. In fact, we show that if these previous models are trained and tested on images taken from positions away from such fixed locations, the reconstruction performance drops significantly. Besides, many real-world applications such as UAV acquisition and underwater acquisition can have images from arbitrary locations and requiring them to obtain images from a particular viewpoint may be infeasible.

To mitigate this inconsistency and to increase the robustness of chosen camera positions, we render images from a much broader viewpoint. We use PyTorch3D \cite{pytorch3d} to render images from much broader viewpoints with Soft Phong Shader. We choose elevations of $-90^{\circ}, -60^{\circ}, -30^{\circ}, 0^{\circ}, 30^{\circ}, 60^{\circ}, 90^{\circ}$ and the azimuths also vary uniformly around the sphere to generate 24 views that span the whole view sphere to represent a real acquisition scenario. Also, some of the object textures are incompatible with PyTorch3D and thus, we use those models without adding any default texture. This choice also adds robustness to both textured and untextured images. We finally use 11 views in this experiment, since diametrically opposite images are degenerate for untextured images (images from both poles are also removed to maintain mathematical stability during rendering calculations). A schematic representation of the camera locations is provided in Figure \ref{fig:overview-model}.
%The number of viewpoints decrases from either side of equator to account for decreasing spatial distance between two points at same azimuth. 

To evaluate the performance of our proposed model on real images, we use the Pix3D dataset \cite{pix3d}. Pix3D offers real-world images of common objects, along with a 3D model of the same. The images are accompanied with mask for the respective object class. There are multiple images corresponding to one 3D object taken from various viewpoints. Although viewpoint-mapping is not provided explicitly, we use the camera position of the input image metadata and map it to the nearest viewpoint used in the previous synthetic data. However, we observe that the dataset does not contain as many images to cover the whole viewpoint. In such a scenario, the next-best view is the one which has the highest probability out of the available viewpoints.

\subsection{Evaluation Metrics}
We use the standard Intersection over Union (IoU) as the evaluation metrics. As the name suggests, this metric is the ratio of number of matching occupied voxels and the total number of occupied voxels. Mathematically,
\begin{equation}
   IoU = \frac{\sum\limits_{\forall x, \forall y, \forall z} \mathbbm{1}_{\{r_{(x,y,z)}>v_t\}} \land t_{(x,y,z)} }{ \sum\limits_{\forall x \forall y \forall z} \mathbbm{1}_{r_{(x,y,z)}>v_t} \lor t_{(x,y,z)} }
\end{equation}

Here $v_t$ denotes the binarization threshold and $\land$, $\lor$ denote logical AND and OR, respectively. Also, $r_{(x,y,z)}$ and $t_{(x,y,z)}$ denotes values at location $(x,y,z)$ for predicted voxel grid and ground truth, respectively. IoU ranges from 0 to 1, with higher value implying better reconstruction.

\subsection{Network Parameters}
We use PyTorch \cite{pytorch_paper} to train 3D-NVS described in the previous section. The network is trained until convergence which takes about 30 hours on an Nvidia 1080Ti GPU. The number of epochs is set to 20 with a batch size of 8. The learning time per epoch is high due to an increased number of gradient calculations for one sample. For all the possible next views, the model parameters are shared and hence the network computes gradients for all the images. Fortunately, it also leads to a considerable increase in learning per epoch. The learning rate of the network layers is set to 0.0001. We experiment with both SGD optimizer and Adam optimizer \cite{kingma:adam} and report the latter due to a better performance. We use standard data augmentation techniques like adding random jitter and using random colored background for better robustness. To recall, the input images are of size 228x228 and the output shape is a voxel grid of size 32x32x32.

\begin{figure*}
\begin{center}
\includegraphics[scale=0.22]{figures/final_v7.pdf}
\end{center}
   \caption{Examples of rendered input images and corresponding reconstruction performance. The images are sorted according to the probability outputs of NVS-Net. The voxel grids below them represents the reconstruction performance with that view along with the input image. We see a good reconstruction for high probability views and the performance decreases as we choose less probable next views, showing that the selected next view is indeed the best. (zoom-in to compare voxel grids).}
\label{fig:sample_ouputs}
\end{figure*}

\subsection{Reconstruction Evaluation}
\label{sec:synthetic-results}
\subsubsection{Synthetic Multi-view Images}
To establish the effectiveness of our approach, we compare the reconstruction performance on various state of the art shape reconstruction methods. We conduct the experiment on rendered images discussed in Section \ref{sec:dataset}. Also, we again train 3D-NVS on the limited-elevation rendered images used in Pix2Vox \cite{pix2vox}, 3D-R2N2 \cite{3dr2n2} and Yang et. al \cite{yang2018active} for a fair baseline and to demonstrate the robustness of our model with respect to capturing locations.

A comparison of our results with that of 3D-R2N2 and Pix2Vox is included in Table \ref{tab:result}. All the methods are trained on our rendered images with a wider viewing angles and a mix of textured and untextured images. The proposed 3D-NVS  achieves a mean IoU of 0.601, thus outperforming both Pix2Vox and 3D-R2N2 which achieves a mean IoU of 0.574 and 0.511 respectively. This improvement in 3D-NVS is due to a better selection of the second view, given the first input image. On the other hand, both Pix2Vox and 3D-R2N2 chooses a fixed set of views for two-view reconstruction -- thus not learning subsequent views. An illustration of reconstructed shapes is provided in Figure \ref{fig:sample_ouputs} where we also show reconstructed shapes when we choose $i^{th}$ view for $i>1$. We can observe that for 3D-NVS we obtain a good reconstruction (IoU $\approx$ 0.80) while the shape degrades as we choose less probable next views.

Next, we use the texture-rich, limited-elevation rendered images used in Pix2Vox, 3D-R2N2 and Yang et. al and trained our model on that rendered images. We obtain a mean IoU of 0.651 which is better than two-view reconstruction in 3D-R2N2 (0.607) and Yang et. al (0.636) and less than Pix2Vox (0.686).

In conclusion, we see that 3D-NVS outperforms all the other methods in both reconstruction using images captured from spread-out viewpoints and the ability to generalize to different input image settings. When moving from a texture-rich, limited-elevation data to a spread-out viewpoint, the performance of Pix2Vox and 3D-R2N2 drops by 11\% and 9\% respectively. In contrast, this decrease in performance is only 5\% in 3D-NVS. We could not compare results in Yang et. al on our rendered images due to unavailability of open-sourced, reproducible code. Most of the other state of the art techniques use range cameras with depth map for reconstruction or view selection and comparison with those methods is not relevant since 2D images contains much less information than RGBD images.
%We compare our work with 3D-R2N2 \cite{3dr2n2} and Pix2Vox \cite{pix2vox} and tabulate the results in Table \ref{tab:result}. We obtain a mean IoU of 0.601 which outperforms 3D-R2N2 (0.511) and Pix2Vox (0.574). This improvement of 3D-NVS is due to a better selection of the second view, given the first input image. On the hand, both Pix2Vox and 3D-R2N2 chooses a fixed set of views for two-view reconstruction -- thus not learning the subsequent views. \ka{Can add something more here}. 
We also the compare our view selection method with commonly used baselines in the literature, namely 3D-NVS-R, where we choose next views randomly, and 3D-NVS-F, which is choosing views so as to maximize the spatial distance between camera positions. This choice of view selection is a heuristic widely used in NBV prediction \cite{shapenet,yang2018active,delmerico2018comparison, hashim2019next, ly2019autonomous}. A detailed analysis of the setting and results is included in the Ablation Study (see Section \ref{sec:ablation}). Moreover, we are able to do this in real time unlike traditional methods in NBV prediction which use range sensors and optimize for surface coverage or information gain and take tens of seconds. This high speed of our method is made possible as it only requires a forward pass through the NVS-net and can also be highly parallelized using a GPU.
%In the results presented above we train all the three methods on the same set of rendered images. The rendered images are obtained as described previously in section \blue{??}. These set of input images are spatially spread out compared to the input images used in their respective work. We observe a decrease due to this generalization in Pix2Vox (11\%), 3D-R2N2 (9\%) and our 3D-NBV (6\%). In conclusion, 3D-NBV outperforms the state of the art reconstructions techniques in more generalized viewpoints -- which is representative to image acquisition in many practical scenarios. Also, we perform competitively on image acquisition done on a circular trajectory \sk{numbers? Also we can push this to ablation}.
%\ka{Small paragraph on some other method which is not done by us?}
%\sk{MAjor difference is the dataset, we can just mention that. All others use range cameras someway or the other.}
\subsubsection{Next-View Prediction}
\begin{figure}
\begin{center}
\includegraphics[scale=0.41]{figures/nvs_class_wise.pdf}
\end{center}
   \caption{An example showing locations of next view selected by the proposed method for two object classes aeroplane and chair. For aeroplane class, both best and second best views are majorly above the equitorial position but for chair its indeed the equitorial position, which concurs with surface methods of view selection.}
\label{fig:next-view-pattern}
\end{figure}

One of the advantage of our 3D-NVS over other previous methods is that we do not require ground-truth for next view selection despite it being posed as a classification problem. Consequently, our method learns this selection on the fly using supervision from 3D shape. It is expected that for some classes of objects, viewing from a particular position is generally more informative than some other viewpoints. For example, consider the class aeroplane. If we view aeroplane from equitorial plane, a significantly less area is captured in the image. Thus, it is less likely that the chosen next view will lie on the equitorial plane. Rather, viewing from an elevation will be more informative. Now consider the class chair. It is intuitive that the maximum area is exposed when it is viewed from an equitorial plane. 

3D-NVS is able to learn this class-specific next view selection without explicit characterization. We illustrate this effect with two example classes as shown in Figure \ref{fig:next-view-pattern}. For both the classes, we choose a fixed position for base image. Next, we observe the number of best and second-best selection of NVS-Net in the test dataset which we denote as 3D-NVS and 3D-NVS-II respectively. As expected, we observe that for both aeroplane and chair classes, NVS is based on the 3D shape of the object. These observations are in conjunction with works that use range images and choose views to maximize the surface area that is scanned by the sensor reinforcing the effectiveness of 3D-NVS.
\vspace{-2mm}
\subsubsection{Real Images}
We also test our model on real images from the Pix3D dataset. We generate a mapping of next views as described previously in section \ref{sec:dataset}. We encounter some missing images as Pix3D consists of common items and the images are taken from typical standing positions. Thus, we choose the next view based on the best NVS-Net output for which a mapping of next image exists. Denoting $Y$ as the output of NVS-Net and $A$ as a boolean vector corresponding to available viewpoints, the next view selection is 
\begin{equation}
   \argmax_i A_i Y_i
\end{equation}
We do not separately train the network again on real images unlike in Pix3D \cite{pix3d}, 3D-R2N2 \cite{3dr2n2} and Pix2Vox \cite{pix2vox}. 3D-NVS achieves an IoU of 0.105 while randomized view selection (NVS-R) achieves an IoU of 0.08. A similar performance is obtained in Pix2Vox when a model trained on synthetic images is used. Thus, we see that using NVS-Net for next view prediction improves the performance on real images even without an explicit training for such images. Therefore, 3D-NVS learns to better generalized on unseen data and seem to be better at scene understanding.
%\sk{we can say here that the 3D-NVS better learns the 3D reconstruction process and generalizes well to unseen data compared to others.}

\subsection{Ablation Study}
\label{sec:ablation}
In this section, we discuss the performance comparison when certain parts of 3D-NVS is replaced with other view selection method to show the effectiveness of our network. 
\subsubsection{Individual Sub-network Performance}
Our proposed 3D-NVS selects the next view based on features extracted from the base image. In contrast, some of the earlier work uses camera position as a parameter to select the next view. We show that if NVS-net is removed and replaced with these heuristics the performance decreases.

We use two methods for view selection : random next view (3D-NVS-R) and farthest next view (3D-NVS-F), both are widely used baseline in NBV prediction \cite{shapenet,yang2018active,delmerico2018comparison, hashim2019next, ly2019autonomous}. In the former, given any input image, we choose the next image randomly from all the available views. On the other hand, for farthest next view, we incorporate the knowledge of camera position and find out the next view which is spatially the farthest. In both the cases, we observe that the mean reconstruction IoU is significantly less than the IoU obtained when using NVS-net output to select the next views. The results are presented in Table \ref{tab:result}.

Another important feature of 3D-NVS is the Context-Aware Fusion followed by Refiner. We again observe that if we replace these sub-parts and replace with simple average of coarse volumes the performance decreases substantially. These findings are in coherence with the findings of Pix2Vox \cite{pix2vox} and hence, we omit a numerical comparison.
\vspace{-1mm}
\subsubsection{View selection orders}
During testing, the NVS-Net gives a softMax output which is the probability distribution over next views. The next view with the highest probability is selected as the next best view. Now, to investigate if the NVS-Net indeed outputs the best possible view selection, we modify the network to choose the $i^{th}$-best view ($i>1$) and compare the results with NVS-Net. All the other parts of the network are kept the same.
We observe a decrease in mean IoU of the reconstruction as we increase $i$. The results are plotted in Figure \ref{fig:ablation} and an example of reconstructed shapes is given in Figure \ref{fig:sample_ouputs}. This decrease in performance when we deter from the selection of the NVS-Net implies that NVS-Net is indeed effective in selecting the next view.

\begin{figure}
\begin{center}
\includegraphics[scale=0.42]{figures/ablation.pdf}
\end{center}
   \caption{A comparison of 3D-NVS reconstruction performance with sub-optimal view selections. 3D-NVS-II denotes second best view is selected, and so on.  }
\label{fig:ablation}
\end{figure}
%\subsection{Individual stage performance}
%\sk{Here we show performance of the model by chipping away blocks for instance: only reconstruction network performance, without fusion-refiner stages.}
